On the Learnability of Deep Random Networks

In this paper we study the learnability of deep random networks from both theoretical and practical points of view. On the theoretical front, we show that the learnability of random deep networks with sign activation drops exponentially with its depth. On the practical front, we find that the learnability drops sharply with depth even with the state-of-the-art training methods, suggesting that our stylized theoretical results are closer to reality.

==> OLD.tex <==
\section{A repulsion property}

In this section we prove a basic property of random deep networks.  The key point is that whatever be the initial angle between the pair of inputs $x, y$, after a few random $i$ layers, the vectors $x^{(i)}, y^{(i)}$ quickly become close to orthogonal.  Specifically the distribution of the angle becomes indistinguishable from the case had the inputs been chosen randomly.

For the remainder of this section we fix a pair of inputs $x$ and $y$ that are not collinear and study the behavior of a random network on both these inputs.  Let $\theta_i = \theta(x^{(i)}, y^{(i)})$ denote  the angle between the outputs at layer $i$ and let $c_i = \cos(\theta_i)$.  Our goal is to study the evolution of $c_i$ as a function of $i$.

Recall that the $j$th bit of $x^{(i)}$, namely 
$x^{(i)}_j$, is obtained by taking  $\sgn(W^{(i)}_j \cdot x^{(i-1)})$, where $W^{(i)}_j$ is the $j$th row of $W^{(i)}$.  Similarly, 
$y^{(i)}_j = \sgn(W^{(i)}_j \cdot y^{(i-1)})$.
We now calculate the expected value of the product of the bits of $x^{(i)}$ and $y^{(i)}$.
%
\begin{lemma}
\label{lem:recur}
For any $i$ and any $j \leq n$, it holds that
$E[x^{(i)}_j y^{(i)}_j] = \mu(c_{i-1})$.
\end{lemma}
%
\begin{proof}

Applying Lemma~\ref{lem:hyperplane} to $x^{(i)}$ and $y^{(i)}$ with $W^{(i)}_j$ as the random vector, we obtain
\begin{eqnarray}
E[x^{(i)}_j y^{(i)}_j] & = & -1 \cdot \frac{\theta_{i-1}}{\pi} + 1 \cdot \left(1 - \frac{\theta_{i-1}}{\pi} \right) = 1 - \frac{2 \theta_{i-1}}{\pi} \nonumber \\
& = & \frac{2}{\pi} \left( \frac{\pi}{2} - \arccos c_{i-1} \right) \nonumber \\
& = & \frac{2}{\pi} \arcsin c_{i-1} = \mu(c_{i-1}). \nonumber
\qedhere
\end{eqnarray}
\end{proof}

We now measure the expected angle between $x^{(i)}$ and $y^{(i)}.$  Note that $c_i \sim \Bern(n, \mu(c_{i-1}))$.
%
\begin{corollary}
\label{cor:recur}
$E[c_i~\mid~c_{i-1}] = \mu(c_{i-1}).$
\end{corollary}
%
\begin{proof}
Taking the expectation of
\begin{equation}
\label{eqn:ci}
c_i = \cos(\theta_i) = \frac{ \sum_{j} x^{(i)}_j y^{(i)}_j}{\|x\| \|y\|},
\end{equation}
applying Lemma~\ref{lem:recur}, and using $\|x\| = \|y\| = \sqrt{n}$ finishes the proof.
\end{proof}
%
To proceed, we next introduce the following definition.
%
\begin{definition}[$(\epsilon, d)$-mixing]
A pair of inputs $x, y$ is \emph{$(\epsilon, d)$-mixed} if the difference between the mean of $c_d(x, y)$ and the mean of $c_d(x', y')$, where $x', y'$ are chosen uniformly at random in $\{ \pm 1 \}^n$, is at most $\epsilon$.
\end{definition}
%
Our goal is to show that $x, y$ is mixed by studying the stochastic iteration defined by Corollary~\ref{cor:recur}.    Note that by symmetry, $E[c_d(x', y')] = 0$.  Hence, to show $(\epsilon, d)$-mixing, it suffices to show $|E[c_d(x, y)]| \leq \epsilon$.  We will in fact show that the iterative process $(\exp(-d), d)$-mixes for $d$ sufficiently large.

\newcommand{\CM}{\mathcal{M}}

\subsection{Mixing using random walks}

Corollary~\ref{cor:recur} states a stochastic recurrence for $c_i$; it is a Markov process, where for each $i > 0$, $c_i \sim \Bern(n, \mu(c_{i-1}))$.  However the recurrence is non-linear and hence it is not straightforward to analyze.  Our analysis will consist of two stages.  In the first stage, we will upper bound the number of steps $d$ such that with overwhelming probability $|c_d|$ goes below a sufficiently small constant.  In the second stage, we will condition that $|c_i|$ is below a small constant (assured by the first stage) and define a modified stochastic process that dominates the original process but is easier to analyze.  

Note that $c_i$ can take at most $2n+1$ distinct values since the inner product between a pair of $\pm 1$ vectors takes only discrete values $-n$ through $n$.  This leads to interpreting the recurrence in Corollary~\ref{cor:recur} as a random walk on a $(2n+1)$-node graph.  (A minor issue is that there are two sink nodes corresponding to $+1$ and $-1$.  We will argue that as long as the inputs are not collinear, the probability of ending up in one of these sink nodes is exponentially small.)

We now begin with the first stage of the analysis.
%
\begin{lemma}
\label{lem:first}
For $d = O(\log \log n)$, we have
\[
\Pr[|c_d| > \mu_0] \leq d \cdot \exp(-\Omega(\sqrt n)).
\]
\end{lemma}
%
\begin{proof}
For ease of understanding let us assume $c_0 \ge 0$; an analogous argument works for the negative case.

For convenience, we will track $\epsilon_i = 1 - c_i$ and show that $1 - \epsilon_i$ rapidly goes to a value bounded away from 1.  Initially, 
$\epsilon_0 \geq 1/n$ since the Hamming distance between $x$ and $y$, which are not collinear, is at least $1$.  

From Corollary~\ref{cor:recur} and Lemma~\ref{lem:useful}(i), we have for $i \geq 1$,
\[
E[1 - \epsilon_i ~\mid~ c_{i-1}] = \mu(1 - \epsilon_{i-1}) \leq 1 - \frac{1}{\pi} \sqrt{2\epsilon_{i-1}},
\]
equivalently,
\[
E[\epsilon_i ~\mid~ \epsilon_{i-1}] \geq \frac{1}{\pi} \sqrt{2 \epsilon_{i-1}}.
\]
This implies by a Chernoff bound that for any $i \geq 1$,
\begin{eqnarray*}
\Pr \left[ \epsilon_i < \frac{1}{2 \pi} \sqrt{2 \epsilon_{i-1}} ~\mid~ \epsilon_{i-1} \right]
& \geq & e^{-\Omega(E[\epsilon_i ~\mid~ \epsilon_{i-1}] \cdot n)} \\
& = & e^{-\Omega(\sqrt{\epsilon_{i-1}} \cdot n)}.
\end{eqnarray*}
If the above high probability event keeps happening for $d = O(\log \log n)$ steps, then $\epsilon_i$ will keep increasing and
$c_i = 1 - \epsilon_i$ will become less than $\mu_0$ in $d$ steps.  Further, the probability that any of these high probability events do not happen is, by a union bound, at most $\sum_{i = 1}^d e^{-\Omega(\sqrt{\epsilon_{i-1}} \cdot n)}
\leq d \cdot e^{-\Omega(\sqrt{n})}$ since each $\epsilon_i \geq 1/n$.
\end{proof}

We now move to the second stage.  For the rest of the section we will work with the condition that $|c_i| < \mu_0$ for all $i > d$, where $d$ is given by Lemma~\ref{lem:first}.   First we bound the probability that $c_i$ continues to stay small $h$ steps after $d$.
%
\begin{lemma}
\label{lem:cont}
For $h > 0$, $\Pr[\exists i \in [d, d+h]: |c_i| > \mu_0 ~\mid~ |c_d| < \mu_0] \leq h e^{-\Omega(n)}$.
\end{lemma}
%
\begin{proof}
If $|c_{i-1}| \le \mu_0$, $\Pr[|c_i| > \mu_0 ~\mid~ c_{i-1}] \le e^{-\Omega(n)}$ from a Chernoff bound as in the proof of Lemma~\ref{lem:first}.  A union bound finishes the proof.
\end{proof}
%
From Lemma~\ref{lem:useful}(ii), we know that for $|c| \leq \mu_0$, we have $|\mu(c)| \leq \rho |c|$.  We use this to define a modified Markov process for $i > d$: $c'_i \sim \Bern(n, \mu'(c'_{i-1}))$, where $\mu'(x) = \rho x$ and we let $c'_d = c_d$.  We will compare our Markov process to the modified process.  To do this, we need a stochastic dominance property.
%
\begin{lemma}
\label{lem:dom}
If $|c_d| = |c'_d| < \mu_0$, then for all $i \geq d$, as long as each successive $|c_i| \leq \mu_0$, we have $|\Bern(n, \mu(c_i))| \preceq |\Bern(n, \mu'(c'_i))|$.
\end{lemma}
%
\begin{proof}
Using Lemma~\ref{lem:sd} and Lemma~\ref{lem:useful}(ii), if $|c_d| = |c'_d| \leq \mu_0$, then for $i > d$, we have $|\Bern(n, \mu(c_i))| \preceq |\Bern(n, \mu'(c'_i))|$.

Since $c_{i+1} \sim \Bern(n, \mu(c_i))$ and using the fact that $\mu$ and $\mu'$ are monotone, and $\mu(x) \leq \mu'(x)$, we can
iteratively apply the above reasoning to complete the proof.
\end{proof}
%
The modified Markov process, however, is easier to analyze.  
%
\begin{lemma}
\label{lem:second}
If $|c_d| \le \mu_0$, then for all $h > 0$, we have
$
|E[c_{d+h} ~\mid~ c_d]| \le \mu_0 \rho^h + h e^{-\Omega(n)}.
$
\end{lemma}
%
\begin{proof}
By the definition of the modified process, using an induction, we have
\[
|E[c'_{d+i} ~\mid~ c'_d| = \rho^i |c'_d| \leq \mu_0. 
\]
The proof now follows from the fact that the Markov process is dominated by the modified process (Lemma~\ref{lem:dom}) except when $c_i$ exceeds $c$ which happens with a small probability as given by Lemma~\ref{lem:cont}.
\end{proof}
%
From Lemma~\ref{lem:first} and Lemma~\ref{lem:second}, we 
conclude the following.
%
\begin{corollary}
For any $x, y$ not collinear we have $|E[c_{d+h}]| \le e^{-\Omega(h)} + h e^{-\Omega(n)} + d e^{-\Omega(\sqrt n)} $. 
\end{corollary}

\section{Learnability}
\label{sec:theory}

In this section we discuss the implications of the repulsion property we showed in Section~\ref{sec:repul}.

\subsection{Statistical correlations}

We will now show that the statistical correlation of the network $f_{w_h}(x)$ (parameterized by $w_h$)  with some fixed function $g(x)$ is exponentially small in the depth $h$ of the network is small for a random $w$. Let us pick all the input vectors $x$ that are on on in one halfspace: this ensures that no two inputs are colinear -- there are $N = 2^{n-1}$ such inputs. $|g|_p = E_x [g(x)^p]^{1/p}$. This will imply that for a typical network $w_h$, we will not be able to detect any correlation $<f_w(x),g(x)>$ with some fixed function $g(x)$. 

\begin{lemma}
$
E_w [ E_x[g(x) f_w(x)]^2 ] 
 \le (1/N) |g|_2^2 + |g|_1^2 exp(-h)
$. This is $exp(-\Omega(h))$ for $g$ with bounded first and second norm and when $h < n$
\end{lemma}
\begin{proof}

\begin{eqnarray}
&
E_w [ E_x[g(x) f_w(x)]^2 ] 
\\
= & (1/N)^2  (\sum_x E_w[g(x)^2 f_w(x)^2] + 2 \sum_{x_1,x_2} E_w[g(x_1) g(x_2) f_w(x_1) f_w(x_2)])
\\
= & (1/N^2) \sum_x g(x)^2  + (1/N^2) (2 \sum_{x_1,x_2} g(x_1) g(x_2) E_w [f_w(x_1) f_w(x_2)])
\\
\le & (1/N) E_x[g(x)^2]  + exp(-h) (1/N^2)  (2 \sum_{x_1,x_2} |g(x_1)| |g(x_2)| 
\\
\le & (1/N)  |g|_2^2   + exp(-h) |g|_1^2
\end{eqnarray}
\end{proof}

\subsection{Statistical Query Hardness}
The statistical query model introduced by Kearns \cite{Kea93} is a natural restriction of the
PAC learning model in which a learning algorithm cannot see labelled examples of the
target concept, but instead may only estimate probabilities involving the target concept.
Formally, when learning with respect to distribution D the learning algorithm is given access
to STAT(f,D)–a statistical query oracle for target concept $F$ with respect to distribution
D. A query to this oracle is a pair $(\Psi, r)$, where $ψ : {0, 1}n × {−1, +1} → {−1, +1}$ is a
query function and r ∈ [0, 1] is a real number called the tolerance of the query. The oracle
may respond to the query with any value v satisfying
|ED[ψ(x, f(x))] − v| ≤ r .
We denote the result returned by oracle STAT(f,D) to query (ψ, r) by STAT(f,D)[ψ, r].
We say that the concept class F is (strongly) learnable from statistical queries (SQ–
learnable) if there is a learning algorithm A, and polynomials p(·, ·, ·), q(·, ·, ·) and r(·, ·, ·)
such that for every $n, f \in F$, distribution $D$ and  the following holds. Given n, the size s of
f,  and access to STAT(f,D), algorithm A produces an –approximation to f with respect
to D in time bounded by p(n, s, 1/). Furthermore, algorithm A makes queries (ψ, r) in
which ψ can be evaluated in time bounded3 by q(n, s, 1/), and in which r is lower-bounded
by 1/r(n, s, 1/).

We start by showing a simple property of statistical queries which simplifies the analysis
of the SQ model. According to the definition of statistical query, the query function ψ is a
Boolean function of two parameters. The first one is denoted by x and the second one is
denoted by f(x) according to the values substituted when estimating the expectation of the
query function. We distinguish two types of statistical queries (either regular or extended)
based on their query function. We say that a query is independent of the target if it is
based on ψ which is a function of x alone (and does not depend on the value of the second
parameter – f(x)) and we say that a query is correlational if φ(x, f(x)) ≡ g(x)f(x) for a
Boolean function g(x).
\begin{lemma} [from feldman]
Any statistical query (regular or extended) can be substituted by two statistical
queries that are independent of the target and two correlational queries.
\end{lemma}

A query that is independent of the target is estimation of the expectation of random
variable which is independent of f and therefore such a query can be substituted by a call
to procedure AMEAN (we assume that the learning algorithm is able to sample randomly with
respect to the distribution of the query). Thus we may assume that learning algorithms in
the statistical query based models use only the correlational statistical queries

We say that W –approximates V with respect to distribution D if for every
f ∈ V there exists g ∈ W such that g –approximates f with respect to distribution D. For
a concept class F denote by Fs the set of all the functions in F of size s.

\begin{theorem}[from feldman]
Theorem 31 Let F be a concept class weakly SQ–learnable with respect to D, particularly, there exists an algorithm A that for every f ∈ Fs, uses at most p(n, s) queries of
tolerance lower-bounded by 1
r(n,s) to produce ( 1
2 − 1
q(n,s) )–approximation to f. Let r
(n, s)
max{2r(n, s), q(n, s)}. There exists a collection of sets {Wi}∞
i=1 such that |Ws| ≤ p(n, s)+1
and Ws ( 1
2 − 1
r(n,s) )–approximates Fs with respect to D.
\end{theorem}

\begin{corollary}
If  $
E_{f\in F} [ E_x[g(x) f(x)]^2 ] < \le (1/N) |g|_2^2 + |g|_1^2 exp(-h)$, our class of functions $F_s$ is not SQ-learnable unless $p\times q > \exp{h}$
\end{corollary}

\subsection{An upper Bound}

We will now show that a random network of depth $h$ can be learn't upto accuracy $e^{-O(h)}$. In fact we show that it can be learn't by a linear function.

\begin{lemma}
A random network of depth $h$ can be learn't upto accuracy $e^{-O(h)}$
\end{lemma}

Let $W_1 .. W_h$ denote the layers of the random network with sign activations in each layer. We will show that the linear function $y_h(x) = W_h.. W_1 x$ is highly correlated with $f_h(x) = \sigma(W_h (\sigma (W_{h-1} .. \sigma (W_1 x))))$. We will show this by induction. Let $q_h$ denote $E[y_h(x).f_h(x)]$

\begin{lemma}
$E[q_h] = e^{-O(h)}$
\end{lemma}
\begin{proof}
Let $y$ and $z$ denote the  vector of outputs at depth $h-1$ and $\tilde y$ and $\tilde z$ are their normalized versions. If $\theta$ is the angle between them then $\cos\theta = \tilde y . \tilde z$.
Now 
$y_h = \sigma(Wy)$ and $f_h = Wz$

Now $E[y_h .f_h] = \sum_i E[\sigma(w_i.y) (w_i.z)]$
   
Let $\theta$ be the angle between $y$ and $z$. Then we can write $\tilde z = \tilde y \cos\theta + y_{\perp} \sin\theta$.
Since $w = w_i$ is distributed as $N(0,1/n)^n$,  
$$
E[\sigma(w_i.y) (w_i.z) = |y||z|E[(w.\tilde y)(w.\tilde y \cos\theta + w.y_{\perp} \sin \theta)]
$$
So 
$$
E[y_h .f_h]  = |y||z|n (E[(w.\tilde y)^2 \cos\theta] +  E[(w.\tilde y)(w.\tilde y_{\perp}) \sin \theta)])
$$

The second part in the sum is zero and the first part is $\rho \cos \theta / n$  for some constant $\rho$. So the total sum is
$
|y||z| \rho \cos \theta
= |y||z| \rho \tilde y. \tilde z
= \rho y.z
$
So $E[y_h.f_h ] = \rho E[y_{h-1} f_{h-1}]$
So $E[y_h .f_h] = \rho^h E[y_0 f_0] = \rho^h n$
So $E[y_h .f_h/n] = \rho^h$
\end{proof}

\section{$k$-way Independence}
Next we will show that the outputs are $k$-way independent for $k = O(\sqrt n)$. Our version of $k$-way independence will be somewhat relaxed:

\begin{definition}
$\eps$-additive-close to full independence: A set of $k$ bits is fully independent if the probability of seeing a specific combination of values is  $1/2^k$. It is $\eps$ close to fully independent if its probability distribution differs from the fully independent distribution in statistical distance by at most $\eps$.
\end{definition}

\begin{definition}
$\eps$-additive-close to   $k$-way independence: A binary function is $\eps$-additive-close to $k$-way independent if the outputs any $k$ inputs is $\eps$-additive-close to fully independent.
\end{definition}

\begin{definition}
$(1 \pm \eps)$-multiplicative-close to full independence: A set of $k$ bits $1 \pm \eps$ factor close to independent if the probability of seeing a specific combination of values is  $(1 \pm \eps).1/2^k$.
\end{definition}

Now take a subset of $k$ binary inputs $x$ so that no pair is equal to one another or opposite; that is, $x_i \ne \pm x_j$.
We will also exclude opposites among the $k$ inputs.

\begin{theorem}
The function $f$ with depth $\Omega (\log n)$ is $\tilde O(k^2/\sqrt{n})$-additive close to $k$-way-independent
\end{theorem}

\begin{theorem}
For a function $f$ of depth $d = \Omega (\log n)$, with high probability of $1-1/poly(n)$ over the first $d-1$ layers, the output after the last layer is $e^{\pm \tilde O(k^2/\sqrt{n})}$-multiplicative close to fully independent. 
\end{theorem}


\begin{observation}
If $k$ outputs at a layer $i$ are orthogonal then after one layer the outputs $y_{i+1}$ form a set of $k$ fully independent $n$ dimensional vectors.
\end{observation}

The main idea behind the following lemma is that the $k$ outputs become near orthogonal after $\Omega(\log n)$ layers. 

\begin{lemma}
The above Markov process $1/poly(n)$ mixes in $O(\log n)$ steps. After this many steps $|c_i| = O(\sqrt{\log s/n})$ with probability $1-1/s$ 
\end{lemma}
\begin{proof}
Assume $c_0$ is at most some constant $c < 1$. Note that w.h.p. $c_i$ is concentrated around $E[c_i]$.

Lets look at the recurrence for the expected value: $E[c_i] = (2/pi) \sin^{-1}(c_{i-1}) \le \rho  c_{i-1}$ for some constant $\rho < 1$ as long as $c_{i_1} \le c < 1$. So then $E[c_i] \le \rho E[c_{i-1}]$. So after $O(\log n)$ steps $E[c_i] = O(1/poly(n))$.

Even if initial value is $1 - \eps$. Then after one iteration the
value becomes $(\pi - 2\cos^{-1}(1-\eps))/\pi = 1 - (2/\pi) \Omega(\sqrt \eps)$. Note that the recurrence $1-\eps_i = 1 - (2/\pi)  \Omega(\sqrt \eps_{i-1})$ quickly goes to a value bounded away from $1$.

So w.h.p. $1- \log n/s$, after $O(\log n)$ steps, $c_i = \pm O(\sqrt{\log s/n})$. 
\end{proof}

\begin{corollary}
For $N$ inputs, w.h.p. after $O(\log n + \log N)$ layers, all pairs from the set of $N$ inputs have mixed.
\end{corollary}

\begin{claim}
If $k$ inputs to a layer are near orthogonal that if the normalized dot products are $\pm \delta$ then after one layer any one column of outputs is $e^{\pm \delta n^2}$-multiplicative close to independent.
\end{claim}
\begin{proof}
We are dotting the $k$ inputs with a random vector $w$ and then taking sign. If $X$ denotes the matrix formed by these inputs as rows, then lets look at the distribution of $y = X w$. If rows of $X$ were orthogonal, $y$ is a uniform gaussian random vector in $R^k$. If $X$ is near orthogonal, it will depart slightly from a uniform gaussian. Lets look at the p.d.f.

$y$ is also $k$ dimensional normally distributed vector with $k \times k$ covariance matrix $U = XX'$.

So p.d.f. of $y$ will be $c.1/\sqrt{det(U)} e^{-x'U^{-1}x}$. If all the normalized dot products are at most $\delta$. Then $U = I + \Delta$ where each entry in $\Delta$ is at most $\delta$. So eigenvalues of $U$ is at most $1 \pm \delta k$. So the determinant is $e^{\pm \delta k^2}$. So over all the distribution differs from that of a uniform normal distribution by a factor of $e^{\pm \delta k^2}$.
\end{proof}

Since w.h.p. $1 - 1/poly(n)$ the normalized dot product is $\pm \sqrt{\log n / n}$, we know that conditioned on this, we get a $1+k^2 \sqrt{\log n/n}$-multiplicative close to fully independent outputs. So over all it is $O(k^2 \sqrt{\log n / n})$-additive-close to fully independent. This gives.

\begin{theorem}
The function $f$ after depth $\Omega(\log n)$ is $O(k^2/poly(n))$-additive close to $k$-way-independent 
\end{theorem}

\section{Extending to Relu}
We now extend the previous analysis of the sign activation function to the RELU activation function. As in the previous analysis, the key step is to show that whatever be the initial angle between the pair of inputs $x, y$, after a few random $i$ Relu layers, the vectors $x^{(i)}, y^{(i)}$ quickly become close to orthogonal.
Recall that for the RELU (and sigmoid) teacher networks, to keep the output vectors at each layer bounded, we normalize and mean-shift every layer's output (This is analogous to applying batch normalization at each layer - we refer to this function as $B$). Thus, the operation at each layer is the following: 1) Multiply the previous layer's outputs by a random Gaussian matrix $W$. 2) Apply RELU 3) Apply batch normalization
As before, we fix a pair of input vectors $x_i$ and $y_i$ with unit length and inner product $c_0$ and study the behavior of this RELU layer on the inner product $c_1$ of the corresponding output vectors.
In particular, we are interested in $E_W(c_{i+1} | c_i} = E_W(c(x_{i+_1}, y_{i+1}))$. This can be written as $E_W(c(B(Relu(W \dot x_i)\dot B(Relu(W \dot x_i)))$. By stability of Gaussians and since $W$ is a random gaussian matrix, $W \dot x_i$ and $W \dot y_i$ are also Gaussian random vectors. Hence we have the following lemma
\begin{lemma}
$E_W(c(x_{i+_1}, y_{i+1})) = E_{x,y \in \mathcal{N(0,1)}, c(x,y) = c_i}[B(Relu(x) \dot B(Relu(y))]$
\end{lemma}

We make the following simplifying assumption in our analysis (based on the Central Limit Theorem):
\begin{assumption}
Assumption: The output of applying RELU activation to a random Gaussian vector, followed by multiplication by a random Gaussian matrix is also Gaussian distributed. This is essentially invoking the Central Limit Theorem since by applying the assumption layer by layer, the output of each RELU Layer is IID (though not Gaussian, but a truncated Gaussian). 
\end{assumption}
Thus, we need to analyze how the angle between two Gaussian vectors changes when passed through each layer, which comprises of the following steps: 
1) Apply RELU
2) Apply batch normalization
3) Multiply by random Gaussian matrix

Assume we have two vectors $x_1, x_2$ at angle $\theta$ and dot product $c_0=cos(\theta)$. Lets find the expected dot product between the vectors ($c_1$) after applying one iteration. Since multiplying by a random Gaussian matrix does not change the expected dot product, we can ignore step 3 of the iterative process. Furthermore, since all dimensions are independent, WLOG we can analyze the angle for one dimension. Thus, we are interested in the following:

$E(q(\sigma(x_1)), q(\sigma(x_2)))$, where $q$ is the batch-normalization operator. This is the same as 
$E(c_1) = E(q(\sigma(x)), q(\sigma(cos(\theta)x + sin(\theta)y)))
= E(q(\sigma(x)), q(c_0 x + sqrt(1 - c_0^2)y)))$, where x and y are IID gaussian variables. 

Figure~\ref{fig1} shows the plot of the above expected value of $c_1$ as a function of $c_0$. As long as $|c_0|$ is bounded away from 1, this value is decreasing by a constant factor. We note that the variance can be handled just as in the sign case above. Thus, under the above assumption we get the following claim.

\begin{figure}
 \centering
 \includegraphics[angle=270,scale=0.3]{plot.pdf}
 \caption{Ratio of $c_1/c_0$}
 \label{figure:relu}
\end{figure}


\begin{claim}
Under the assumption, for RELU, for any $x_1,x_2$ that are sufficiently far from identical $|E[y_{i,1} y_{i,2}]| \le exp(-i)$
\end{claim}

\section{Extending to Relu2}
We now extend the previous analysis of the sign activation function to the RELU activation function. As in the previous analysis, the key step is to show that whatever be the initial angle between the pair of inputs $x, y$, after a few random $i$ Relu layers, the vectors $x^{(i)}, y^{(i)}$ quickly become close to orthogonal.
Recall that for the RELU (and sigmoid) teacher networks, to keep the output vectors at each layer bounded, we normalize and mean-shift every layer's output (This is analogous to applying batch normalization at each layer - we refer to this operator as $B(.)$). Thus, the operation at each layer is the following: 1) Multiply the previous layer's outputs by a random Gaussian matrix $W$. 2) Apply RELU 3) Apply batch normalization.
As before, we fix a pair of input vectors $x_i$ and $y_i$ with length $\sqrt{n}$ and inner product $c_0$ and study the behavior of this RELU layer on the inner product $c_1$ of the corresponding output vectors.
In particular, we are interested in $E_W[c_{i+1} | c_i] = E_W[c(x_{i+_1}, y_{i+1})] = E_W[c(B(Relu(W x_i),  B(Relu(W y_i))]$. By stability of Gaussians and since $W$ is a random gaussian matrix, $W x_i$ and $W y_i$ are also Gaussian random vectors. Hence we have the following lemma
\begin{lemma}
$E_W[c_{i+1} | c_i] = E_{x,y \in \mathcal{N}(0,1)^n, c(x,y) = c_i}[c(B(Relu(x)),  B(Relu(y)))]$
\end{lemma}

Thus, we need to analyze how the angle between two random Gaussian vectors changes when passed through a Relu and a Batch normalization operator.
In particular, given two vectors $x, y \in \mathcal{N}(0,1)^n$ at angle $\theta$ and cosine similarity $c_0=cos(\theta)$,  we wish to find the expected cosine similarity ($c_1$) after applying one iteration. Furthermore, since all dimensions of $x$ and $y$ are independent, using an argument similar to that in Corollary \ref{cor:recur}) we have $E_W[c_{i+1} | c_i] = E_{x,y \in \mathcal{N}(0,1), x.y = c_i}[B(Relu(x)) . B(Relu(y))]$. Thus, without loss of generality, we can consider the expected dot product along only one dimension of the Gaussian vectors after applying the Relu and a Batch normalization operator.

In particular, we make the following claim
\begin{claim}
\label{claim:relu1}
$E_{x,y \in \mathcal{N}(0,1), c(x,y) =c_0} [B(Relu(x)) . B(Relu(y))] <= c_0$
\end{claim}

While we do not have an analytical proof for this claim, in Figure~\ref{relu}, we plot this expected value (which we denote as $c_1$) via simulations as a function of $c_0$, which shows that this ratio is always less than 1.  Thus, under the above claim we get the following lemma (analogous to Corollary~\ref{cor:recur} for the sign function).

\begin{figure}
 \centering
 \includegraphics[angle=270,scale=0.3]{plot.pdf}
 \caption{Ratio of $c_1/c_0$}
 \label{figure:relu}
\end{figure}


\begin{lemma}
For the Relu activation function, $E[c_i | c_{i-1}] < c_{i-1}$
\end{lemma}

\begin{proof}
We have
$c_i = \cos(\theta_i) = \frac{ \sum_{j} x^{(i)}_j y^{(i)}_j}{\|x\| \|y\|}$.
Taking expectations on both sides and using the fact that each dimension of $x_i$ and $y_i$ are independent, we have $E[c_i | c_{i-1}] = E[x^{(i)}_j y^{(i)}_j] < 1$, where the last inequality follows from Claim ~\ref{claim:relu1}
\end{proof}

As in the sign case, we define $G(n,p)$ to denote the distribution of the average of $n$ independent random variables  each of which has mean $p$ and is obtained by taking the product of two truncated (as a result of Relu) Gaussian random variables. We have $c_i \sim G(n, \nu(c_{i-1}))$, where we define $\nu(t) = E_{x,y \in \mathcal{N}(0,1), c(x,y) = t} [B(Relu(x)) . B(Relu(y))]$

By Claim~\ref{claim:relu1}, we have $\nu(t) < 1$. As before, we bound the above Markov process by another modified process : $c'_i \sim G(n, \nu'(c'_{i-1}))$, where $\nu'(x) = \psi x$ for some constant $\psi < 1$.  We will compare our Markov process to the modified process using the following stochastic dominance property, similar to that in Lemma ~\ref{lem:dom}.

\begin{lemma}
\label{lem:relu_dom}
For all $i \geq d$, we have $|G(n, \nu(c_i))| \preceq G(n, \nu'(c'_i))|$.
\end{lemma}

Using this stochastic dominance property we have the following lemma
\begin{lemma}
\label{lem:relu-second}
For all $h > 0$, we have
$
|E[c_{h} ~\mid~ c_0]| \le \mu_0 \psi^h$
\end{lemma}
%
\begin{proof}
From the definition of the modified process and by using a simple induction, we obtain
\[
|E[c'_{i} ~\mid~ c'_0| = \psi^i |c'_0| \leq \mu_0 \psi^h. 
\]
The proof now follows from the fact that the Markov process is dominated by the modified Markov process (Lemma~\ref{lem:dom}).
\end{proof}
%
From Lemma~\ref{lem:relu-second}, we 
conclude the following.
%
\begin{theorem}
\label{thm:relu-repulsion}
For any $x, y$ not collinear we have $|E[c_{h}]| \le e^{-\Omega(h)}$. 
\end{theorem}


==> app.tex <==
\section{Stochastic dominance}
\label{sec:sd}

\begin{proof}[Proof of Lemma~\ref{lem:sd}]
We first prove some simpler statements.  Let $X(p)$ denote a random variable that is $+1$ with probability $(1 + p)/2$ and $-1$ otherwise; here $p$ is the \emph{bias}.  
%
\begin{lemma}
\label{lem:sd1}
Let $p_1, \ldots, p_n$ be non-negative biases and let $Y = \sum_{i=1}^n X(p_i)$.  Then, $\Pr[Y = -k-\ell] \leq \Pr[Y = k-\ell]$ for any $k > 0, \ell \geq 0$.
\end{lemma}
\begin{proof}
We show this by an induction on $n$. Clearly the statement is true for $n=0$.  Assume the statement holds for up to $n$.  We will show that the statement holds for the extreme cases $Y + X(0)$ and $Y + 1$ separately.  Since the distribution of $Y + X(p_{n+1})$ is a convex combination of the two it must hold for that as well.

To see that it holds for $Y + 1$, note that 
\[
\Pr[Y + 1 = -k - \ell] - \Pr[Y + 1 = k-\ell]
\enspace = \enspace \Pr[Y = -k - \ell-1] - \Pr[Y = k-\ell-1]
\enspace \le \enspace 0,
\]
by the induction hypothesis.

To see that it holds for $Y + X(0)$, let $U \sim X(0)$; note $U$ is a uniform $\pm 1$ random variable.  Now,  
\begin{eqnarray*}
\Pr[Y + U = -k - \ell] - \Pr[Y + U = k-\ell]
& = & \frac{1}{2} (\Pr[Y = -k -\ell-1] - \Pr[Y = k-\ell-1]) \\
& & \enspace + \enspace \frac{1}{2} (\Pr[Y = -k -\ell+1] - \Pr[Y = k-\ell+1]).
\end{eqnarray*}
%
If $\ell > 0$ the proof is complete by induction.  Otherwise we have $\ell = 0$ and by rearranging the terms above, we obtain 
\[
\frac{1}{2} (\Pr[Y = -k -1] - \Pr[Y = k+1])
\enspace + \enspace \frac{1}{2} (\Pr[Y = -k+1] - \Pr[Y = k-1])
\enspace \leq \enspace 0,
\]
once again by induction.
\end{proof}

\begin{lemma}
\label{lem:sd2}
Let $p_1, \ldots, p_n$ be non-negative biases, let $Y = \sum_i X(p_i)$, and let $0 \leq q \leq r$.  Then we have
$|X(q) + Y| \preceq |X(r) + Y|$.
\end{lemma}
\begin{proof}
To show stochastic dominance, we need to show $\Pr[|X(r) + Y| \ge k] \ge \Pr[|X(q) + Y| \ge k]$,
for all $k$.  We will show the complement, i.e., $\Pr[|X(q) + Y| \le k] \ge \Pr[|X(r) + Y| \le k]$.
Now,
\begin{eqnarray*}
\Pr[|X(q) + Y| \leq k] 
& = & \Pr[X(q) = 1] \cdot \Pr[ -k-1 \leq Y \leq k-1] \\
& & \mbox{} +  \Pr[X(q) = -1] \cdot \Pr[ -k+1 \leq Y \leq k+1] \\
& = &  \frac{1+q}{2} \cdot \Pr[ -k-1 \leq Y \leq k-1] 
+ \frac{1-q}{2}\cdot \Pr[ -k+1 \leq Y \leq k+1] \\
& = & \frac{1+q}{2} \cdot \Pr[ -k-1 \leq Y \leq -k] 
+ \frac{1-q}{2} \cdot \Pr[k \leq Y \leq k+1] \\
& & \mbox{} + \Pr[ -k+1 \leq Y \leq k-1].
\end{eqnarray*}
%
Using this and $q \leq r$, we obtain
\begin{eqnarray*}
\lefteqn{
\Pr[|X(q) + Y| \leq k]  -  \Pr[|X(r) + Y| \leq k]} \\
& = & \frac{q-r}{2} \cdot \Pr[-k-1 \leq Y \leq -k] 
- \frac{q-r}{2} \cdot \Pr[k \leq Y \leq k+1] \\
& = & \left(\frac{q-r}{2}\right) \left( (\Pr[Y = -k-1] + \Pr[Y = -k]) \right. 
- \left(\Pr[Y = k] + \Pr[Y=k+1]) \right) \\
& = & \left(\frac{q-r}{2}\right) \left( (\Pr[Y = -k-1] - \Pr[Y = k+1]) \right.
\left. + (\Pr[Y = -k] - \Pr[Y = k]) \right) \enspace \geq \enspace 0, 
\end{eqnarray*}
using Lemma~\ref{lem:sd1} with $\ell = 0$.
\end{proof}

The proof now follows from applying  Lemma~\ref{lem:sd2} repeatedly over each of the $n$ random variables replacing $X(p)$ by $X(q)$.
\end{proof}

==> leanability.old.before.bug.tex <==
\newcommand{\STAT}{{\sf STAT}}
\newcommand{\SQ}{\mathsf{SQ}}
\newcommand{\CF}{\mathcal{F}}

\section{Learnability}
\label{sec:learnability}

In this section we discuss the implications of the repulsion property we showed in Section~\ref{sec:repulsion}.  We first calculate the statistical correlation of the function computed by a random network with some fixed function.  We use the correlation bound to argue that random networks are hard to learn in the statistical query model.  Finally we show an almost matching converse to the hardness result:  we show upper bounds on the learnability of a random network.

\subsection{Statistical correlations}

We will now show that the statistical correlation $f_{W, h}(\cdot)$, for random $W$, with any fixed function $g(\cdot)$ is exponentially small in the depth $h$ of the network.  Consider all the inputs $x \in \{ \pm \}^n$ that are in one halfspace; this ensures that no two inputs are collinear.   Note that the number of such inputs is $N = 2^{n-1}$.  Define for $p \geq 1$, the norm $|g|_p = E_x[|g(x)|^p]^{1/p}$. 
%
\begin{lemma}
\label{lem:corr}
$E_W [ E_x[g(x) f_{W, h}(x)]^2 ] 
 \le |g|_2^2/N + |g|_1^2 e^{-h}$. 
\end{lemma}
\begin{proof}
\begin{eqnarray*}
\lefteqn{
E_W [ E_x[g(x) f_W(x)]^2 ]
} \\
& = & \frac{1}{N^2} \left( \sum_x E_W[g(x)^2 f_W(x)^2] \right. \\
& & \quad \left. + 2 \sum_{x \neq y} E_W[g(x) g(y) f_{W, h}(x) f_{W, h}(y)] \right)
\\
& = & \frac{1}{N^2} \sum_x g(x)^2  + \frac{2}{N^2} \sum_{x \neq y} g(x) g(y) E_W [f_{W, h}(x) f_{w, h}(y)]
\\
& \le & \frac{1}{N} E_x[g(x)^2] + e^{-h} \frac{2}{N^2} \sum_{x \neq y} |g(x)| |g(y)| 
\\
& \le & \frac{1}{N}  |g|_2^2   + e^{-h} |g|_1^2,
\end{eqnarray*}
using Theorem~\ref{thm:repulsion}.
Note that this bound is $e^{-\Omega(h)}$ when $g$ has bounded first and second norms and when $h = o(\sqrt{n})$.
\end{proof}

\subsection{Statistical query hardness}
\label{sec:sq}

In this section we show how the statistical correlation bound we obtained in Lemma~\ref{lem:corr} leads to hardness of learning in the statistical query (SQ) model.  The SQ model captures many classes of powerful machine learning algorithms including gradient descent, PCA, etc; see for example the survey by \citet{vitaly}.

We briefly recap the \emph{SQ model}~\cite{Kearns98,Bshouty2a}.  In this model, instead of working with labeled examples, a learning algorithm can estimate probabilities involving the target concept.  Let $X$ denote the space of inputs.  Formally speaking, a statistical query oracle $\SQ_{f, D}(\psi, r)$ for a Boolean function $f: X \rightarrow \{\pm 1\}$ with respect to a distribution $D$ on $X$ takes as input a query function $\psi : X \times \{-1, +1\} \rightarrow [-1, +1]$ and a tolerance $r$ and returns $v$ such that $|E_D[\psi(x, f(x))] - v| \leq r$.  A concept class $\CF$ is \emph{SQ-learnable} with respect to a distribution $D$ if there is an algorithm $\mathcal{A}$ that, for every $f \in \CF$, obtains an $\epsilon$-approximation%
\footnote{
A function $f$ is an \emph{$\epsilon$-approximation} to $g$ with respect to $D$ if $\Pr_D[f(x) = g(x)] \geq 1 - \epsilon$.
}
to $f$ with respect to $D$ in time $p(n, s, 1/\epsilon)$ for some polynomial $p(\cdot)$.  Here $n$ is the number of parameters to describe any $x \in X$ and $s$ is the number of parameters to describe any $f \in \CF$.  We assume that the evaluation of the function that $\mathcal{A}$ uses for the $\SQ_{f, D}$ oracle takes time $q(n, s, 1/\epsilon)$ and the tolerance is $1/r(n, s, 1/\epsilon)$, where $q(\cdot)$ and $r(\cdot)$ are also polynomials.

It has been shown that for Boolean functions, the statistical query function $\psi$ can be restricted to be a \emph{correlation query} function of the form $\psi(x, f(x)) = g(x) f(x)$, where $g(x) \in [-1, 1]$.  The following can be inferred from Lemma~12 and the arguments in Section~5.1 in \citet{Bshouty2a}.
%
\begin{lemma}
\label{lem:sq2corr}
For Boolean function $f$, all statistical queries made by an SQ-learning algorithm can be restricted to be correlational queries.
\end{lemma}
%
%Let $\CF^s$ denote the subset of $\CF$ of size $s$.
%
\begin{theorem}[\citet{Bshouty2a}, Theorem~31]
\label{thm:vitaly}
Let $\CF$ be a concept class that is SQ-learnable with respect to $D$, particularly, there exists an algorithm $\mathcal{A}$ that for every $f \in \CF$, uses at most $p(n, s)$ queries of tolerance lower bounded by $1/r(n,s)$ to produce a $(1/2 - 1/q(n,s))$-approximation to $f$. Let $r'(n, s) = \max\{ 2r(n, s), q(n, s) \}$.  There exists a collection of sets $\{ W_i  \}_{i = 1}^{\infty}$ such that $|W_s| \leq p(n, s)+1$ and the set $W_s$ $(1/2 - 1/r'(n,s))$-approximates%
\footnote{
A set $W$ \emph{$\epsilon$–approximates} $F$ with respect to distribution $D$ if for every $f \in F$ there exists $g \in W$ such that $g$ $\epsilon$-approximates $f$ with respect to $D$.
}
$\CF$ with respect to $D$.
\end{theorem}
%
Using these, we now show the hardness result.
%
\begin{theorem}
\label{thm:hardness}
If  $E_{f \in \CF} [ E_D [g(x) f(x)]^2 ] < \epsilon(n, s)$, then the class $F^s$ of functions is not SQ-learnable unless $p(n, s) \cdot \max(r(n, s), q(n, s))^2 > 1/\epsilon(n, s)$.
\end{theorem}
%
\begin{proof}
\rknote{This proof needs rewrite}
Given that the square of the correlation of a uniformly chosen random function $f \in \CF$ is at most $\epsilon$, by a Markov bound, with probability $1 - 1/p(n, s)$, the correlation with a fixed $g$ will also be at most $p(n, s)  \cdot \epsilon(n, s)$.   By a union bound, the correlation squared with all the functions in $W_s$ will then be at most $O(p(n, s) \cdot \epsilon(n, s))$;  i.e., the absolute value of the correlation is $O(\sqrt{p(n, s) \cdot \epsilon(n, s)})$.  However, for the desired tolerance and learnability in Theorem~\ref{thm:vitaly}, there is a function $g \in W_s$ such that $g$ $(1/2 - 1/r'(n, s)$-approximates $f$, i.e., the correlation of $g$ with $f$ is $1/r'(n, s)$.  Thus, we need
$O(\sqrt{p(n, s) \cdot \epsilon(n, s)}) \geq 1/r'(n, s)$, which completes the proof.
\end{proof}
%
In our case, will use $h$ instead of $s$ to parameterize the target class.  Since $g(x) \in [-1, 1]$, $|g|_1 \leq 1$ and the following SQ lower bound follows then follows from Lemma~\ref{lem:corr} and Theorem~\ref{thm:hardness}.

\begin{theorem}
\label{thm:sqhardnessdeepnetwork}
For any SQ algorithm for learning a random deep network of depth $h$
$p(n, h) \cdot \max(r(n, h), q(n, h))^2 > e^{O(h)}$. In particular this means that to get accuracy that is a constant better than $1/2$, the number of queries $p$ is exponential in $h$; If the number of queries is $poly(h)$ then the improvement over an accuracy of $1/2$ is $exp(-h)$.
\end{theorem}

In the next section, we will show a matching upper bound of $exp(-h)$  for the achievable accuracy in polynomial time.
\subsection{An upper bound}
\label{sec:lb}

We will now show that $f_{W, h, \sigma}$, i.e., a random network of depth $h$ with $\sigma$ activation, can indeed be learned up to an accuracy of $e^{-O(h)}$, in fact, by a linear function.  This essentially complements the hardness result in Section~\ref{sec:sq}.  

We will show that the linear function defined by $g_{W, h}(x) = W^{(h+1)} W^{(h)} \cdots W^{(1)} x$ is highly correlated with $f_{W, h, \sigma}(x)$. We complete the proof by induction.
%
\begin{lemma}
$E[g_{W, h}(x) \cdot f_{W, h, \sigma}(x)] = e^{-O(h)}$.
\end{lemma}
\begin{proof}
\rknote{Does this work for all $\sigma$?}
We study the output at each layer for both $f$ and $g$.  Let $y$ (resp., $z$) denote the vector of inputs to the $h$th layer of $f_{W, h, \sigma}(x)$ (resp., $g_{W, h}(x)$).  Let $\hat{y} = y / \|y\|$ and $\hat{z} = z / \|z\|$; note that $\|y\| = \sqrt{n}$ for $\sigma = \sgn$.  If $\theta = \theta(y, z)$, then we have 
$\cos(\theta) = \hat{y} \cdot \hat{z}$.  Now,
%
\begin{eqnarray}
\lefteqn{
\mkern-36mu E_W[f_{W, h, \sigma}(x) \cdot g_{W, h}(x)] = 
\sum_i E[\sigma(W^{(h)}_i \cdot y) (W^{(h)}_i \cdot z)]} \nonumber \\
& = & \|z\| \sum_i E_W[\sigma(W^{(h)}_i \cdot y) (W^{(h)}_i \cdot \hat{z})].  \label{eq:ub1}
\end{eqnarray}
%
The key step is to express $\hat{z} = \hat{y} \cos\theta + y_{\perp} \sin\theta$.  Fix an $i$ and for brevity let $w = W^{(h)}_i$.  Since $w \sim N(0,1/n)^n$,  we obtain
\begin{eqnarray}
\lefteqn{
E_w[\sigma(w \cdot y) (w \cdot \hat{z})]} \nonumber \\
&  = & E[\sigma(w \cdot y) \left(w \cdot \hat{y} \cos\theta +  w \cdot y_{\perp} \sin \theta \right)] \nonumber \\
& = & E[\sigma(w \cdot y)(w \cdot \hat{y}) \cos\theta] 
+  E[\sigma(w \cdot y) (w \cdot y_{\perp}) \sin \theta] \nonumber \\
& = & E[\sigma(w \cdot y)(w \cdot \hat{y})] \cos\theta 
+  E[\sigma(w \cdot y)] E[w \cdot y_{\perp}] \sin \theta \nonumber \\
& = &\frac{\cos \theta}{\sqrt{n}} E[\sigma(w \cdot y)(w \cdot y)] 
+  E[\sigma(w \cdot y)] E[w \cdot y_{\perp}] \sin \theta \nonumber \\
& = & \frac{\gamma}{\sqrt{n}} \cos \theta. \label{eq:ub2}
\end{eqnarray}
%
Here, the third equality follows since the random variables $w \cdot y$ and $w \cdot y_{\perp}$ are independent.  The fourth equality follows since $\|y\| = \sqrt{n}$.  The final equality follows since (i) $w \cdot y \sim \|y\| N(0, 1/n) \sim N(0, 1)$ and hence the expectation in the first term is of the form $E_r[\sigma(r) \cdot r]$ where $r \sim  N(0, 1)$, which is some absolute constant%
\footnote{
For $\sigma = \sgn$, $\gamma$ is the mean of the folded unit normal distribution and is  $\sqrt{2/\pi} \approx 0.8$.
} $\gamma < 1$ that depends on $\sigma$
and
(ii) the second term vanishes since 
$w \cdot y_{\perp} \sim \| y_{\perp} \| N(0, 1/n)$.
Plugging (\ref{eq:ub2}) into (\ref{eq:ub1}), we obtain
\begin{eqnarray*}
\lefteqn{
E_W[f_{W, h, \sigma}(x) \cdot g_{W, h}(x)] = \|z\| \cdot n \cdot \frac{\gamma}{\sqrt{n}} \cos \theta} \\
& = &  \|y\| \|z\| \cdot \gamma \cos \theta 
\enspace = \enspace \|y\| \|z\| \cdot \gamma (\hat{y} \cdot \hat{z}) \\
& = & \gamma (y \cdot z) 
\enspace = \enspace \gamma^h n,
\end{eqnarray*}
by an induction on $h$ and using the base case at the input layer where $x \cdot x = n$.  
Since the final output of $f_{W, h, \sigma}$ is a bit, the average correlation with $g_{W, h}$ is $\gamma^h = e^{-O(h)}$.
\end{proof}


==> learnabilityold.tex <==
\newcommand{\STAT}{{\sf STAT}}
\newcommand{\SQ}{\mathsf{SQ}}
\newcommand{\CF}{\mathcal{F}}

\section{Learnability}
\label{sec:learnability}

In this section we discuss the implications of the repulsion property we showed in Section~\ref{sec:repulsion}.  We first calculate the statistical correlation of the function computed by a random network with some fixed function.  We use the correlation bound to argue that random networks are hard to learn in the statistical query model.  Finally we show an almost matching converse to the hardness result:  we show upper bounds on the learnability of a random network.

\subsection{Statistical correlations}

We will now show that the statistical correlation $f_{W, h}(\cdot)$, for random $W$, with any fixed function $g(\cdot)$ is exponentially small in the depth $h$ of the network.  Consider all the inputs $x \in \{ \pm \}^n$ that are in one halfspace; this ensures that no two inputs are collinear.   Note that the number of such inputs is $N = 2^{n-1}$.  Define for $p \geq 1$, the norm $|g|_p = E_x[|g(x)|^p]^{1/p}$. 
%
\begin{lemma}
\label{lem:corr}
$E_W [ E_x[g(x) f_{W, h}(x)]^2 ] 
 \le |g|_2^2/N + |g|_1^2 e^{-h}$. 
\end{lemma}
\begin{proof}
\begin{eqnarray*}
\lefteqn{
E_W [ E_x[g(x) f_W(x)]^2 ]
} \\
& = & \frac{1}{N^2} \left( \sum_x E_W[g(x)^2 f_W(x)^2] \right. \\
& & \quad \left. + 2 \sum_{x \neq y} E_W[g(x) g(y) f_{W, h}(x) f_{W, h}(y)] \right)
\\
& = & \frac{1}{N^2} \sum_x g(x)^2  + \frac{2}{N^2} \sum_{x \neq y} g(x) g(y) E_W [f_{W, h}(x) f_{w, h}(y)]
\\
& \le & \frac{1}{N} E_x[g(x)^2] + e^{-h} \frac{2}{N^2} \sum_{x \neq y} |g(x)| |g(y)| 
\\
& \le & \frac{1}{N}  |g|_2^2   + e^{-h} |g|_1^2,
\end{eqnarray*}
using Theorem~\ref{thm:repulsion}.
Note that this bound is $e^{-\Omega(h)}$ when $g$ has bounded first and second norms and when $h = o(\sqrt{n})$.
\end{proof}

\subsection{Statistical query hardness}
\label{sec:sq}

In this section we show how the statistical correlation bound we obtained in Lemma~\ref{lem:corr} leads to hardness of learning in the statistical query (SQ) model.  The SQ model captures many classes of powerful machine learning algorithms including gradient descent, PCA, etc; see for example the survey by \citet{vitaly}.

We briefly recap the \emph{SQ model}~\cite{Kearns98,Bshouty2a}.  In this model, instead of working with labeled examples, a learning algorithm can estimate probabilities involving the target concept.  Let $X$ denote the space of inputs.  Formally speaking, a statistical query oracle $\SQ_{f, D}(\psi, r)$ for a Boolean function $f: X \rightarrow \{\pm 1\}$ with respect to a distribution $D$ on $X$ takes as input a query function $\psi : X \times \{-1, +1\} \rightarrow [-1, +1]$ and a tolerance $r$ and returns $v$ such that $|E_D[\psi(x, f(x))] - v| \leq r$.  A concept class $\CF$ is \emph{SQ-learnable} with respect to a distribution $D$ if there is an algorithm $\mathcal{A}$ that, for every $f \in \CF$, obtains an $\epsilon$-approximation%
\footnote{
A function $f$ is an \emph{$\epsilon$-approximation} to $g$ with respect to $D$ if $\Pr_D[f(x) = g(x)] \geq 1 - \epsilon$.
}
to $f$ with respect to $D$ in time $p(n, s, 1/\epsilon)$ for some polynomial $p(\cdot)$.  Here $n$ is the number of parameters to describe any $x \in X$ and $s$ is the number of parameters to describe any $f \in \CF$.  We assume that the evaluation of the function that $\mathcal{A}$ uses for the $\SQ_{f, D}$ oracle takes time $q(n, s, 1/\epsilon)$ and the tolerance is $1/r(n, s, 1/\epsilon)$, where $q(\cdot)$ and $r(\cdot)$ are also polynomials.

It has been shown that for Boolean functions, the statistical query function $\psi$ can be restricted to be a \emph{correlation query} function of the form $\psi(x, f(x)) = g(x) f(x)$, where $g(x) \in [-1, 1]$.  The following can be inferred from Lemma~12 and the arguments in Section~5.1 in \citet{Bshouty2a}.
%
\begin{lemma}
\label{lem:sq2corr}
For Boolean function $f$, all statistical queries made by an SQ-learning algorithm can be restricted to be correlational queries.
\end{lemma}
%
Let $\CF^s$ denote the subset of $\CF$ of size $s$.
%
\begin{theorem}[\citet{Bshouty2a}, Theorem~31]
\label{thm:vitaly}
Let $\CF$ be a concept class that is SQ-learnable with respect to $D$, particularly, there exists an algorithm $\mathcal{A}$ that for every $f \in \CF^s$, uses at most $p(n, s)$ queries of tolerance lower bounded by $1/r(n,s)$ to produce a $(1/2 - 1/q(n,s))$-approximation to $f$. Let $r'(n, s) = \max\{ 2r(n, s), q(n, s) \}$.  There exists a collection of sets $\{ W_i  \}_{i = 1}^{\infty}$ such that $|W_s| \leq p(n, s)+1$ and the set $W_s$ $(1/2 - 1/r'(n,s))$-approximates%
\footnote{
A set $W$ \emph{$\epsilon$–approximates} $F$ with respect to distribution $D$ if for every $f \in F$ there exists $g \in W$ such that $g$ $\epsilon$-approximates $f$ with respect to $D$.
}
$\CF^s$ with respect to $D$.
\end{theorem}
%
Using these, we now show the hardness result.
%
\begin{theorem}
\label{thm:hardness}
If  $E_{f \in \CF^s} [ E_D [g(x) f(x)]^2 ] < \epsilon(n, s)$, then the class $F^s$ of functions is not SQ-learnable unless $p(n, s) \cdot \max(r(n, s), q(n, s))^2 > 1/\epsilon(n, s)$.
\end{theorem}
%
\begin{proof}
\rknote{This proof needs rewrite}
Given that the square of the correlation of a uniformly chosen random function $f \in \CF^s$ is at most $\epsilon$, by a Markov bound, with probability $1 - 1/p(n, s)$, the correlation with a fixed $g$ will also be at most $p(n, s)  \cdot \epsilon(n, s)$.   By a union bound, the correlation squared with all the functions in $W_s$ will then be at most $O(p(n, s) \cdot \epsilon(n, s))$;  i.e., the absolute value of the correlation is $O(\sqrt{p(n, s) \cdot \epsilon(n, s)})$.  However, for the desired tolerance and learnability in Theorem~\ref{thm:vitaly}, there is a function $g \in W_s$ such that $g$ $(1/2 - 1/r'(n, s)$-approximates $f$, i.e., the correlation of $g$ with $f$ is $1/r'(n, s)$.  Thus, we need
$O(\sqrt{p(n, s) \cdot \epsilon(n, s)}) \geq 1/r'(n, s)$, which completes the proof.
\end{proof}
%
In our case, will use $h$ instead of $s$ to parameterize the target class.  Since $g(x) \in [-1, 1]$, $|g|_1 \leq 1$ and our SQ lower bound follows then follows from Lemma~\ref{lem:corr} and Theorem~\ref{thm:hardness}.

\begin{theorem}
\label{thm:sqhardnessdeepnetwork}
For any SQ algorithm for learning a random deep network of depth $h$
$p(n, h) \cdot \max(r(n, h), q(n, h))^2 > e^{O(h)}$. In particular this means that to get accuracy that is a constant better than $1/2$, the number of queries $p$ is exponential in $h$; If the number of queries is $poly(h)$ then the improvement over an accuracy of $1/2$ is $exp(-h)$ 
\end{theorem}

In the next section, we will show a matching upper bound of $exp(-h)$  for the achievable accuracy in polynomial time.
\subsection{An upper bound}
\label{sec:lb}

We will now show that $f_{W, h, \sigma}$, i.e., a random network of depth $h$ with $\sigma$ activation, can indeed be learned up to an accuracy of $e^{-O(h)}$, in fact, by a linear function.  This essentially complements the hardness result in Section~\ref{sec:sq}.  

We will show that the linear function defined by $g_{W, h}(x) = W^{(h+1)} W^{(h)} \cdots W^{(1)} x$ is highly correlated with $f_{W, h, \sigma}(x)$. We complete the proof by induction.
%
\begin{lemma}
$E[g_{W, h}(x) \cdot f_{W, h, \sigma}(x)] = e^{-O(h)}$.
\end{lemma}
\begin{proof}
\rknote{Does this work for all $\sigma$?}
We study the output at each layer for both $f$ and $g$.  Let $y$ (resp., $z$) denote the vector of inputs to the $h$th layer of $f_{W, h, \sigma}(x)$ (resp., $g_{W, h}(x)$).  Let $\hat{y} = y / \|y\|$ and $\hat{z} = z / \|z\|$; note that $\|y\| = \sqrt{n}$ for $\sigma = \sgn$.  If $\theta = \theta(y, z)$, then we have 
$\cos(\theta) = \hat{y} \cdot \hat{z}$.  Now,
%
\begin{eqnarray}
\lefteqn{
\mkern-36mu E_W[f_{W, h, \sigma}(x) \cdot g_{W, h}(x)] = 
\sum_i E[\sigma(W^{(h)}_i \cdot y) (W^{(h)}_i \cdot z)]} \nonumber \\
& = & \|z\| \sum_i E_W[\sigma(W^{(h)}_i \cdot y) (W^{(h)}_i \cdot \hat{z})].  \label{eq:ub1}
\end{eqnarray}
%
The key step is to express $\hat{z} = \hat{y} \cos\theta + y_{\perp} \sin\theta$.  Fix an $i$ and for brevity let $w = W^{(h)}_i$.  Since $w \sim N(0,1/n)^n$,  we obtain
\begin{eqnarray}
\lefteqn{
E_w[\sigma(w \cdot y) (w \cdot \hat{z})]} \nonumber \\
&  = & E[\sigma(w \cdot y) \left(w \cdot \hat{y} \cos\theta +  w \cdot y_{\perp} \sin \theta \right)] \nonumber \\
& = & E[\sigma(w \cdot y)(w \cdot \hat{y}) \cos\theta] 
+  E[\sigma(w \cdot y) (w \cdot y_{\perp}) \sin \theta] \nonumber \\
& = & E[\sigma(w \cdot y)(w \cdot \hat{y})] \cos\theta 
+  E[\sigma(w \cdot y)] E[w \cdot y_{\perp}] \sin \theta \nonumber \\
& = &\frac{\cos \theta}{\sqrt{n}} E[\sigma(w \cdot y)(w \cdot y)] 
+  E[\sigma(w \cdot y)] E[w \cdot y_{\perp}] \sin \theta \nonumber \\
& = & \frac{\gamma}{\sqrt{n}} \cos \theta. \label{eq:ub2}
\end{eqnarray}
%
Here, the third equality follows since the random variables $w \cdot y$ and $w \cdot y_{\perp}$ are independent.  The fourth equality follows since $\|y\| = \sqrt{n}$.  The final equality follows since (i) $w \cdot y \sim \|y\| N(0, 1/n) \sim N(0, 1)$ and hence the expectation in the first term is of the form $E_r[\sigma(r) \cdot r]$ where $r \sim  N(0, 1)$, which is some absolute constant%
\footnote{
For $\sigma = \sgn$, $\gamma$ is the mean of the folded unit normal distribution and is  $\sqrt{2/\pi} \approx 0.8$.
} $\gamma < 1$ that depends on $\sigma$
and
(ii) the second term vanishes since 
$w \cdot y_{\perp} \sim \| y_{\perp} \| N(0, 1/n)$.
Plugging (\ref{eq:ub2}) into (\ref{eq:ub1}), we obtain
\begin{eqnarray*}
\lefteqn{
E_W[f_{W, h, \sigma}(x) \cdot g_{W, h}(x)] = \|z\| \cdot n \cdot \frac{\gamma}{\sqrt{n}} \cos \theta} \\
& = &  \|y\| \|z\| \cdot \gamma \cos \theta 
\enspace = \enspace \|y\| \|z\| \cdot \gamma (\hat{y} \cdot \hat{z}) \\
& = & \gamma (y \cdot z) 
\enspace = \enspace \gamma^h n,
\end{eqnarray*}
by an induction on $h$ and using the base case at the input layer where $x \cdot x = n$.  
Since the final output of $f_{W, h, \sigma}$ is a bit, the average correlation with $g_{W, h}$ is $\gamma^h = e^{-O(h)}$.
\end{proof}


==> repulsion.before.bug.tex <==
\section{A repulsion property}
\label{sec:repulsion}

In this section we prove a basic property of random deep networks.  The key point is that whatever be the initial angle between the pair of inputs $x, y$, after a few random $i$ layers, the vectors $x^{(i)}, y^{(i)}$ become close to orthogonal.  Specifically the distribution of the angle becomes indistinguishable from the case had the inputs been chosen randomly.

For the remainder of this section we fix a pair of inputs $x$ and $y$ that are not collinear and study the behavior of a random network on both these inputs.  Let $\theta_i = \theta(x^{(i)}, y^{(i)})$ denote  the angle between the outputs at layer $i$ and let $c_i = \cos(\theta_i)$.  Our goal is to study the evolution of $c_i$ as a function of $i$.

Recall that the $j$th bit of $x^{(i)}$, namely 
$x^{(i)}_j$, is obtained by taking  $\sgn(W^{(i)}_j \cdot x^{(i-1)})$, where $W^{(i)}_j$ is the $j$th row of $W^{(i)}$.  Similarly, 
$y^{(i)}_j = \sgn(W^{(i)}_j \cdot y^{(i-1)})$.
We now calculate the expected value of the product of the bits of $x^{(i)}$ and $y^{(i)}$.
%
\begin{lemma}
\label{lem:recur}
For any $i$ and any $j \leq n$, it holds that
$E[x^{(i)}_j y^{(i)}_j ~\mid~ c_{i-1}] = \mu(c_{i-1})$.
\end{lemma}
%
\begin{proof}

Applying Lemma~\ref{lem:hyperplane} to $x^{(i)}$ and $y^{(i)}$ with $W^{(i)}_j$ as the random vector, we obtain
\begin{eqnarray}
\lefteqn{
E[x^{(i)}_j y^{(i)}_j ~\mid~ c_{i-1}] = -1 \cdot \frac{\theta_{i-1}}{\pi} + 1 \cdot \left(1 - \frac{\theta_{i-1}}{\pi} \right)} \nonumber \\
& = & 1 - \frac{2 \theta_{i-1}}{\pi} 
\enspace = \enspace \frac{2}{\pi} \left( \frac{\pi}{2} - \arccos c_{i-1} \right) \nonumber \\
& = & \frac{2}{\pi} \arcsin c_{i-1}
\enspace = \enspace \mu(c_{i-1}). \nonumber
\qedhere
\end{eqnarray}
\end{proof}

We now measure the expected angle between $x^{(i)}$ and $y^{(i)}.$  Note that $c_i \sim \Bern(n, \mu(c_{i-1}))$.
%
\begin{corollary}
\label{cor:recur}
$E[c_i~\mid~c_{i-1}] = \mu(c_{i-1}).$
\end{corollary}
%
\begin{proof}
Taking the expectation of
\begin{equation}
\label{eqn:ci}
c_i = \cos(\theta_i) = \frac{ \sum_{j} x^{(i)}_j y^{(i)}_j}{\|x\| \|y\|},
\end{equation}
applying Lemma~\ref{lem:recur}, and using $\|x\| = \|y\| = \sqrt{n}$ finishes the proof.
\end{proof}
%
To proceed, we next introduce the following definition.
%
\begin{definition}[$(\epsilon, d)$-mixing]
A pair of inputs $x, y$ is \emph{$(\epsilon, d)$-mixed} if 
$| E[c_d(x, y)] - E[c_d(x', y')]| \leq \epsilon$, where $x', y'$ are chosen uniformly at random in $\{ \pm 1 \}^n$.
\end{definition}
%
Our goal is to show that $x, y$ is mixed by studying the stochastic iteration defined by Corollary~\ref{cor:recur}.    Note that by symmetry, $E[c_d(x', y')] = 0$.  Hence, to show $(\epsilon, d)$-mixing, it suffices to show $|E[c_d(x, y)]| \leq \epsilon$.  We will in fact show that the iterative process $(\exp(-d), d)$-mixes for $d$ sufficiently large.

\newcommand{\CM}{\mathcal{M}}

\subsection{Mixing using random walks}
\label{sec:mixing}
Corollary~\ref{cor:recur} states a stochastic recurrence for $c_i$; it is a Markov process, where for each $i > 0$, $c_i \sim \Bern(n, \mu(c_{i-1}))$.  However the recurrence is non-linear and hence it is not straightforward to analyze.  Our analysis will consist of two stages.  In the first stage, we will upper bound the number of steps $d$ such that with overwhelming probability $|c_d|$ goes below a sufficiently small constant.  In the second stage, we will condition that $|c_i|, i \geq d$ is below a small constant (assured by the first stage) and define a modified stochastic process that dominates the original process but is easier to analyze.  

Note that $c_i$ can take at most $2n+1$ distinct values since the inner product between a pair of $\pm 1$ vectors takes only discrete values $-n$ through $n$.  This leads to interpreting the recurrence in Corollary~\ref{cor:recur} as a random walk on a $(2n+1)$-node graph.  (A minor issue is that there are two sink nodes corresponding to $+1$ and $-1$.  We will argue that as long as the inputs are not collinear, the probability of ending up in one of these sink nodes is exponentially small.)

We now begin with the first stage of the analysis.
%
\begin{lemma}
\label{lem:first}
For $d = O(\log \log n)$ and $\mu_0$ chosen according to Lemma~\ref{lem:useful}, we have
\[
\Pr[|c_d| > \mu_0] \leq d \cdot \exp(-\Omega(\sqrt n)).
\]
\end{lemma}
%
\begin{proof}
For ease of understanding let us assume $c_0 \ge 0$; an analogous argument works for the negative case.

For convenience, we will track $\epsilon_i = 1 - c_i$ and show that $1 - \epsilon_i$ rapidly goes to a value bounded away from 1.  Initially, 
$\epsilon_0 \geq 1/n$ since the Hamming distance between $x$ and $y$, which are not collinear, is at least $1$.  

From Corollary~\ref{cor:recur} and Lemma~\ref{lem:useful}(i), we have for $i \geq 1$,
\mymath{
E[c_i ~\mid~ c_{i-1}] = \mu(c_{i-1}) = \mu(1 - \epsilon_{i-1}) \leq 1 - \frac{1}{\pi} \sqrt{2\epsilon_{i-1}},
}
equivalently,
\mymath{
E[\epsilon_i ~\mid~ \epsilon_{i-1}] \geq \frac{1}{\pi} \sqrt{2 \epsilon_{i-1}}.
}
This implies by a Chernoff bound that for any $i \geq 1$,
\begin{eqnarray*}
\Pr \left[ \epsilon_i < \frac{1}{2 \pi} \sqrt{2 \epsilon_{i-1}} ~\bigg\vert~ \epsilon_{i-1} \right]
& \geq & e^{-\Omega(E[\epsilon_i ~\mid~ \epsilon_{i-1}] \cdot n)} \\
& = & e^{-\Omega(\sqrt{\epsilon_{i-1}} \cdot n)}.
\end{eqnarray*}
If the above high probability event keeps happening for $d = O(\log \log n)$ steps, then $\epsilon_i$ will keep increasing and
$c_i = 1 - \epsilon_i$ will become less than $\mu_0$ in $d$ steps, where $\mu_0$ is from Lemma~\ref{lem:useful}(ii).  Further, the probability that any of these high probability events do not happen is, by a union bound, at most $\sum_{i = 1}^d e^{-\Omega(\sqrt{\epsilon_{i-1}} \cdot n)}
\leq d \cdot e^{-\Omega(\sqrt{n})}$ since each $\epsilon_i \geq 1/n$.
\end{proof}

We now move to the second stage.  For the rest of the section we will work with the condition that $|c_i| < \mu_0$ for all $i > d$, where $d$ is given by Lemma~\ref{lem:first}.   First we bound the probability that $c_i$ continues to stay small $h$ steps after $d$.
%
\begin{lemma}
\label{lem:cont}
For $h > 0$, $\Pr[\exists i \in [d, d+h]: |c_i| > \mu_0 ~\mid~ |c_d| < \mu_0] \leq h e^{-\Omega(n)}$.
\end{lemma}
%
\begin{proof}
If $|c_{i-1}| \le \mu_0$, $\Pr[|c_i| > \mu_0 ~\mid~ c_{i-1}] \le e^{-\Omega(n)}$ from a Chernoff bound as in the proof of Lemma~\ref{lem:first}.  A union bound finishes the proof.
\end{proof}
%
From Lemma~\ref{lem:useful}(ii), we know that for $|c| \leq \mu_0$, we have $|\mu(c)| \leq \rho |c|$.  We use this to define a modified Markov process for $i > d$: $c'_i \sim \Bern(n, \mu'(c'_{i-1}))$, where $\mu'(x) = \rho x$ and we let $c'_d = c_d$.  We will compare our Markov process to the modified process.  To do this, we need a stochastic dominance property.
%
\begin{lemma}
\label{lem:dom}
If $|c_d| = |c'_d| < \mu_0$, then for all $i \geq d$, as long as each successive $|c_i| \leq \mu_0$, we have $|\Bern(n, \mu(c_i))| \preceq |\Bern(n, \mu'(c'_i))|$.
\end{lemma}
%
\begin{proof}
Since $c_{i+1} \sim \Bern(n, \mu(c_i))$, and using the fact that $\mu$ and $\mu'$ are monotone, and $\mu(x) \leq \mu'(x)$, we can
iteratively apply Lemma~\ref{lem:sd} to complete the proof.
\end{proof}
%
The modified Markov process, however, is easier to analyze.  
%
\begin{lemma}
\label{lem:second}
If $|c_d| \le \mu_0$, then for all $h > 0$, we have
$
|E[c_{d+h} ~\mid~ c_d]| \le \mu_0 \rho^h + h e^{-\Omega(n)}.
$
\end{lemma}
%
\begin{proof}
From the definition of the modified process and by using a simple induction, we obtain
\mymath{
|E[c'_{d+i} ~\mid~ c'_d| = \rho^i |c'_d| \leq \rho^i \mu_0. 
}
The proof now follows from the fact that the Markov process is dominated by the modified Markov process (Lemma~\ref{lem:dom}) except when $c_i$ exceeds $\mu_0$ which happens with a small probability as given by Lemma~\ref{lem:cont}.
\end{proof}
%
From Lemma~\ref{lem:first} and Lemma~\ref{lem:second}, we 
conclude the following.
%
\begin{theorem}
\label{thm:repulsion}
For any $x, y$ not collinear we have $|E[c_{d+h}]| \le e^{-\Omega(h)} + h e^{-\Omega(n)} + d e^{-\Omega(\sqrt n)} $. 
\end{theorem}

\rknote{Account for sink nodes}
